Informative Communication of Robot Plans

When a robot is asked to verbalize its plan it can do it in many ways. For example, a seemingly natural strategy is incremental, where the robot verbalizes its planned actions in plan order. However, an important aspect of this type of strategy is that it misses considerations on what is effectively informative to communicate, because not considering what the user knows prior to explanations. In this paper we propose a verbalization strategy to communicate robot plans informatively, by measuring the information gain that verbalizations have against a second-order theory of mind of the user capturing his prior knowledge on the robot. As shown in our experiments, this strategy allows to understand the robot's goal much quicker than by using strategies such as increasing or decreasing plan order. In addition, following our formulation we hint to what is informative and why when a robot communicates its plan.

==> fig/model.tex <==

\begin{figure}
    \centering

    \begin{tikzpicture}[align=center] 
    \usepgflibrary{shapes.geometric}
    \usetikzlibrary{shapes,backgrounds,shapes.misc, positioning,shapes.geometric,arrows,matrix,fit,calc}
    \tikzstyle{main}=[draw, ellipse, minimum height=1cm, minimum width=1.5cm, align=center]
    
    
    \node[main]                         at (0, 0)    (1) {$B$};
    \node[main]                         at (0, -1.5) (2) {$\Pi$};
    \node[main, fill=lightgray]         at (0, -3)   (3) {$O$};
    \node[draw=white,text width=2cm]    at (0,1.2) {$P_R(B,\Pi,O)$};
    
    \node[main]                         at (5.5, 0)    (4) {$B$};
    \node[main]                         at (5.5, -1.5) (5) {$\Pi$};
    \node[main, fill=lightgray]         at (5.5, -3)   (6) {$O$};
    \node[draw=white,text width=2cm]    at (5.5,1.2) {$P_R^H(B,\Pi,O)$};
    
    \begin{scope}[on background layer]
        \node[draw, thick, rounded corners = 2.5ex, fit=(1) (2),inner sep=3mm, opacity=0.6, fill=orange](Fit1) {};
        \node[draw, thick, rounded corners = 2.5ex, fit=(4) (5),inner sep=3mm, opacity=0.6, fill=red](Fit2) {};
    \end{scope}
    
    
    \draw[->] (1) -- (2);
    \draw[->] (2) -- (3);
    \draw[->] (4) -- (5);
    \draw[->] (5) -- (6);
    
    
    \draw[<->] (Fit1) -- node [midway,above ] {$H(P_R, P_R^H|o)$} (Fit2);
    
        \draw[->] (1) -- (2);


    \end{tikzpicture}
    \caption{Robot model ($P_R$) and second-order theory of mind of the user ($P_R^H$) as equivalent Bayesian Networks. The cross-entropy $H$ measures the difference between robot's and user's estimated state of mind a posteriori of a verbalization $o$. }
    \label{fig:model}
\end{figure}

==> plot/user_study.tex <==

\begin{figure}[H]
    \centering
    \scalebox{.95}{
    \begin{tikzpicture}
    \begin{axis}[
        title={},
        xlabel={\% plan},
        ylabel={Hit ratio},
        xmin=0.1, xmax=1,
        ymin=0, ymax=1,
        xtick={0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1},
        ytick={0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1},
        legend pos=south east,
        ymajorgrids=true,
        grid style=dashed,
        legend entries = {Increasing, Decreasing, Informative},]
    ]
    \addplot[thick,blue] table [x=x, y=increasing, col sep=comma] {data/user_study/hit.csv};
    \addplot[thick,orange] table [x=x, y=decreasing, col sep=comma] {data/user_study/hit.csv};
    \addplot[thick,teal] table [x=x, y=informative, col sep=comma] {data/user_study/hit.csv};
    
        
    \end{axis}
    \end{tikzpicture}
    }

    \caption{Hit ratio of the participants of the user study as a function of percentage of communicated actions.}
    \label{plt:user_study}
\end{figure}

==> table/pucrs.tex <==
\begin{wraptable}{r}{.5\linewidth}
\centering
  \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    \textbf{Domain} & $|\mathcal{P}|$  & $|\mathcal{A}|$  &  $|I|$ & $|G|$ & $|\overline{\pi}|$\\ 
    \hline
    \textit{miconic}	            & 8	    &	4	&	517	    &	6       &	35.57 \\
    \textit{logistics}              & 3	    &	6	&	22.16	&	10.39	&	24.41 \\
    \textit{intrusion}           	& 11	&	9	&	1	    &	16.67	&	13.07 \\
    \textit{blocks-world}        	& 5	    &	4	&	14.58	&	20.28	&	14.50 \\
    \textit{rovers}              	& 32	&	9	&	172.71	&	6       &	24.93 \\
    \textit{satellite}            	& 12	&	5	&	58	    &	6.43	&	16.89 \\
    \hline
  \end{tabular}
    \\[2mm]
  \caption{Average instance measures over the tested planning domains. The columns, from left to right are: number of operators, number of predicates, size of the initial state, number of tested goals, length of optimal plans.}
 \label{tbl:pucrs_dataset}
\end{wraptable}


